DisCo: Remedy Self-supervised Learning on Lightweight Models with Distilled Contrastive Learning

While self-supervised representation learning (SSL) has received widespread attention from the community, recent research argue that its performance will suffer a cliff fall when the model size decreases. The current method mainly relies on contrastive learning to train the network and in this work, we propose a simple yet effective Distilled Contrastive Learning (DisCo) to ease the issue by a large margin. Specifically, we find the final embedding obtained by the mainstream SSL methods contains the most fruitful information, and propose to distill the final embedding to maximally transmit a teacher's knowledge to a lightweight model by constraining the last embedding of the student to be consistent with that of the teacher. In addition, in the experiment, we find that there exists a phenomenon termed Distilling BottleNeck and present to enlarge the embedding dimension to alleviate this problem. Our method does not introduce any extra parameter to lightweight models during deployment. Experimental results demonstrate that our method achieves the state-of-the-art on all lightweight models. Particularly, when ResNet-101/ResNet-50 is used as teacher to teach EfficientNet-B0, the linear result of EfficientNet-B0 on ImageNet is very close to ResNet-101/ResNet-50, but the number of parameters of EfficientNet-B0 is only 9.4\%/16.3\% of ResNet-101/ResNet-50. Code is available at https://github. com/Yuting-Gao/DisCo-pytorch.

==> figures/effib0-r50-r50Effib0-5-15.tex <==
\begin{figure}[ht]
    \centering
    \vspace{-10pt}
    \includegraphics[width=0.9\linewidth]{./figures/effib0-r50-r50Effib0.pdf}
    \vspace{-15pt}
    \caption{Clustering results on the ImageNet test set. Different colors represent different classes. }
    \vspace{-10pt}
    \label{fig:effib0-r50-r50Effib0-5-15}
\end{figure}

==> figures/effib0-r50-r50Effib0.tex <==
\begin{figure*}[tb]
    \centering
    \includegraphics[width=1.0\linewidth]{./figures/effib0-r50-r50Effib0.png}
    \caption{effib0, r50, r50-effib0}
    \label{fig:effib0-r50-r50Effib0}
\end{figure*}

==> figures/limited-labels-2.tex <==
\begin{figure}[ht]
    \centering
    \vspace{-9pt}
    \includegraphics[width=0.37\linewidth]{./figures/limited-labels_2.pdf}
    \vspace{-8pt}
    \caption{ImageNet top-1 accuracy (\%) of semi-supervised linear evaluation.}
    % with 1\%, 10\% and 100\% training data.}
    % Points where the number of teacher network parameters are 0 are the results of the MoCo-V2 without distillation.}
    %The Student models tend to perform better on the semi-supervised tasks after distillation from larger Teachers.}
    % \vspace{-18pt}
    \label{fig:limited-labels_2}
    \vspace{-10pt}
\end{figure}

==> figures/mlp-hidden.tex <==
\begin{figure}[ht]
    \centering
    % \vspace{-5pt}
    \includegraphics[width=0.9\linewidth]{./figures/mlp-hidden.pdf}
    \vspace{-10pt}
    \caption{Linear evaluation top-1 accuracy on ImageNet of student projection head with different dimensions of hidden layer during distillation. $\star$ represents the original dimension used in MoCo-V2.}
    \vspace{-16pt}
    \label{fig:mlp-hidden}
\end{figure}

==> figures/r18-r50w2-r50w2R18.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=1.0\linewidth]{./figures/r18-r50w2-r50w2R18.png}
    \caption{r18-r50w2-r50w2R18}
    \label{fig:r18-r50w2-r50w2R18}
\end{figure*}

==> figures/r34-r101R34-r34.tex <==
\begin{figure*}[tb]
    \centering
    \includegraphics[width=1.0\linewidth]{./figures/r34-r101-r101R34.png}
    \caption{r34, r101, r101-r34}
    \label{fig:r34-r101R34-r34}
\end{figure*}

==> figures/ssl.tex <==
\begin{figure}[ht]
    \centering
    \vspace{-5pt}
    \includegraphics[width=1.0\linewidth]{./figures/ssl.pdf}
    \vspace{-10pt}
    \caption{Diagrams of four mainstream SSL methods.}
    \vspace{-5pt}
    \label{fig:ssl}
\end{figure}

==> figures/transfer-cifar.tex <==
\begin{figure*}[ht]
    \centering
    % \vspace{-5pt}
    \includegraphics[width=1\linewidth]{./figures/transfer-cifar-ar.pdf}
    % \vspace{-23pt}
    \caption{Top-1 accuracy of students transferred to Cifar10/Cifar100 without and with distillation from different teachers.}
    % \vspace{-5pt}
    % Our proposed method (red column) beats SEED (blue column) under various combination of teacher and student models. }
    \label{fig:transfer-cifar}
\end{figure*}

==> figures/transfer-cifar10.tex <==
\begin{figure}[ht]
    \centering
    \vspace{-5pt}
    \includegraphics[width=0.55\linewidth]{./figures/cifar10.pdf}
    \vspace{-15pt}
    \caption{Top-1 accuracy of students transferred to Cifar10.}
    % \caption{Top-1 accuracy of students transferred to Cifar10 without and with distillation from different teachers.}
    \vspace{-15pt}
    \label{fig:transfer-cifar10}
    \vspace{-7pt}
\end{figure}

==> figures/visualization.tex <==
\begin{figure*}[htb]
    \centering
    \includegraphics[width=1.0\linewidth]{./figures/visualization.png}
    \caption{r18, r50, r50-r18}
    \label{fig:visualization}
\end{figure*}

==> sections/method__.tex <==
\section{Related Work}

\subsection{Self-supervised Learning}

SSL is a generic framework that learns high semantic patterns from the data itself without any tags from human beings. Current methods mainly rely on three paradigms, \textit{i.e.},  pretext tasks based, contrastive learning based and clustering based.

\noindent \textbf{Pretext tasks based.} 
Approaches based on pretext paradigm first design surrogate tasks, e.g., Rotation \cite{komodakis2018unsupervised}, Jigsaw \cite{noroozi2016unsupervised}, and then train the network to solve. 

%that identifies whether patches are cropped from the same image, Rotation \cite{komodakis2018unsupervised} that predicts the rotation degree of the input image, and Jigsaw \cite{noroozi2016unsupervised} that places the shuffled patches back to the original position.% and Context encoder \cite{pathak2016context} that recovers the missing part of the input image conditioned on its surrounding.

\noindent \textbf{Contrastive learning based.} Contrastive learning based approaches have shown impressive performance on self-supervised representation learning, which enforce different views of the same input to be closer in feature space \cite{chen2020exploring,chen2020big,chen2020simple,henaff2020data,he2019moco,chen2020mocov2,grill2020bootstrap,wang2020enhancing,wang2020removing}. SimCLR-V2 indicates that SSL can be boosted by applying strong data augmentation, training with larger batch size, and adding projection head after the global average pooling. However, SimCLR relies on a very large batch size to achieve comparable performance. MoCo-V2 considers contrastive learning as a look-up dictionary, using a memory bank to maintain consistent representations of negative samples. Thus, MoCo can achieve superior performance without a large batch size, which is more feasible to implement. 
%BYOL \cite{grill2020bootstrap} introduces a predictor to one branch of the network to break the symmetry and avoid the trivial solution. 
DINO \cite{caron2021emerging} applies contrastive learning to vision transformers.
%Thus, MoCo can stores more negative samples for every sample without large batch size. MoCo can be applied to different model, showing superior performance in most cases.
%Recent works have shown that contrastive learning can be combined with pretext tasks to learn better representation for downstream tasks \cite{pathak2016context,tian2019contrastive}.
% CPC \cite{oord2018representation} classifies the future representation among the unrelated negative set, which is a form of Context encoder~ \cite{pathak2016context}.}
% BYOL~ \cite{grill2020bootstrap} introduces predictor to one branch of the network to break the symmetric for avoiding trivial solution. Although BYOL claims that it doesn't need any negative pairs, BYOL in fact still needs larger batch size to achieve better performance and spends longer time to converge. 
% SimSiam \cite{chen2020exploring} share parameters between two branch and make the whole network more concise. Twins  \cite{zbontar2021barlow} proposes to measure the cross-correlation matrix between the outputs of two identical networks fed with distorted versions of a sample to avoid collapsing. However, it seems that MoCo still the best choice for learning patterns from untagged dataset.

\noindent \textbf{Clustering based.} 
Clustering is a kind of promising approach for unsupervised representation learning \cite{caron2018deep,asano2020self}. 
% Clustering is one of the most promising approaches for unsupervised representation learning. 
%DeepCluster \cite{caron2018deep} uses k-means assignments to generate pseudo-labels to iteratively group the features and update the weight of the network. %DeeperCluster \cite{caron2019unsupervised} scales to large uncurated datasets to capture complementary statistics. % and can be used to pre-train network before supervised tasks. 
%Different from previous works, to maximize the mutual information between pseudo labels and input data, 
%SeLa \cite{asano2020self} cast the pseudo-label assignment as an instance of optimal transport. 
SwAV \cite{caron2020unsupervised} maps representations to prototype vectors and is capable to scale to larger datasets.
% which is assigned online and is capable to scale to larger datasets.

Although mainstream methods SimCLR-V2, MoCo-V2, DINO, and SwAV belong to different self-supervised categories, they have four things in common: 1) two views for each input image, 2) two encoders for feature extraction, 3) two projection heads to map the representations into a lower dimension space, and 4) the two low-dimensional embeddings are regarded as a pair of positive samples and are pulled closer during training, which can be considered as a contrast process. However, all of these methods suffer a performance cliff fall that is way much more severe than expected on lightweight models, which is what we try to remedy in this work.
%\textcolor{red}{Although the mainstream methods SimCLR-V2, MoCo-V2, DINO, and SwAV belong to different self-supervised categories, all of these methods suffer a performance cliff fall on lightweight models, which is what we try to remedy in this work.}

%a model with more parameters will perform better, but a small model with fewer parameters usually fail to achieve comparable performance as well as larger one~ \cite{fang2021seed}.

\subsection{Knowledge Distillation}
Knowledge distillation tries to transfer the knowledge from a larger teacher model to a smaller student model. 
According to the form of knowledge, it can be classified into three categories, logits-based, feature-based, and relation-based. Logits-based method KD \cite{hinton2015distilling} proposes to make the student mimic the logits of the teacher by minimizing the KL-divergence of the class distribution. Feature-based methods \cite{romero2014fitnets,zagoruyko2016paying} directly transfer the knowledge from the intermediate layers of the teacher to student. AT \cite{zagoruyko2016paying} proposes to use the spatial attention of the teacher as the knowledge and let the student pay attention to the area that the teacher is concerned about. Relation-based approaches explore the relationship between data instead of the output of a single instance. RKD \cite{park2019relational} transfers the mutual relationship of the input data within one batch from the teacher to the student. In this work, we use feature-based distillation methods.
%FitNets \cite{romero2014fitnets} regards the intermediate representations learned by the teacher as hints and transfers the knowledge to a thinner and deeper student through minimizing the mean square error between the representations. 

%\noindent \textbf{Logits-based.} Logits refers to the output of the network classifier. KD \cite{hinton2015distilling} proposes to make the student mimic the logits of the teacher by minimizing the KL-divergence of the class distribution. %Logits-based distillation can be further used in different tasks. The output in object detection may contain logits with the offset the bounding box  \cite{chen2017learning}.

%\noindent \textbf{Feature-based.} Feature-based methods directly transfer the knowledge from the intermediate layers of the teacher to student. FitNets \cite{romero2014fitnets} regards the intermediate representations learned by the teacher as hints and transfers the knowledge to a thinner and deeper student through minimizing the mean square error between the representations. AT \cite{zagoruyko2016paying} proposes to use the spatial attention of the teacher as the knowledge and let the student pay attention to the area that the teacher is concerned about. %SemCKD \cite{chen2020cross} adaptively selects the more appropriate representation pairs of the teacher and student. %FSP \cite{yim2017gift} takes the relationship between the intermediate layers of the teacher as the target for the student to mimic.

%\noindent \textbf{Relation-based.} Relation-based approaches explore the relationship between data instead of the output of a single instance. RKD \cite{park2019relational} transfers the mutual relationship of the input data within one batch from the teacher to the student. %IRG \cite{liu2019knowledge} proposes to use the relationship the graph to further express the relational knowledge.

%PKT~ \cite{passalis2018learning} transfer knowledge by matching the probability distribution in feature space instead of feature map representation. 
 
\subsection{SSL meets KD}
% KDSVD used the correlations between features maps 
%KDSVD  \cite{lee2018self} considers the teacher's correlation between features map via singular vector decomposition as supervision for the student network. 

%Recently, some works combine self-supervised learning and knowledge distillation.
%Recently, some knowledge distillation methods \cite{tian2019contrastive, xu2020knowledge} take self-supervision as an auxiliary task to further boost knowledge transfering. 

%CRD \cite{tian2019contrastive} introduces a contrastive loss to transfer pair-wise relationship across different modalities. SSKD\cite{xu2020knowledge} lets the student mimic transformed data and self-supervision tasks to transfer richer knowledge. The above-mentioned works take self-supervision as an auxiliary task to further boost the process of knowledge distillation under fully supervised setting. 
CompRess \cite{koohpayegani2020compress} and SEED \cite{fang2021seed} try to employ knowledge distillation as a means to improve the representation capability of small models in self-supervised learning, which utilize the negative sample queue in MoCo-V2 to constrain the distribution of positive sample over negative samples of the student to be consistent with that of the teacher. However, both methods heavily rely on MoCo-V2, which means that a memory bank has to be preserved during the distillation process. Our method also aims to boost the self-supervised representation learning ability on lightweight models by distilling, however, we do not restrict the self-supervised framework and thus are more flexible. Furthermore, our method surpasses SEED with a large margin on all lightweight models under the same setting.



%, which aims to leverage a larger network (teacher) to transfer its representational knowledge into a smaller architecture (student) in a self-supervised fashion without any labels from human beings. 


==> tables/EI-effect.tex <==
\begin{table}[ht]
    \centering
    \caption{Linear evaluation top-1 accuracy (\%) on ImageNet with SwAV as the testbed.}
    \footnotesize
    \begin{tabular}{ccc}
    \toprule
    	 \textbf{Method} & \textbf{Eff-b0} & \textbf{Mob-v3} \\
    	 \midrule
         SwAV  & 46.8 & 19.4 \\
        %  SwAV + DisCo & 62.4\greenp{15.6$\uparrow$} & 55.7\greenp{36.3$\uparrow$} \\
         SwAV + DisCo & 62.4 & 55.7 \\
        \bottomrule
    \end{tabular}
    \label{tab:EI-effect}
    % \vspace{-10pt}
\end{table}

    % \begin{tabular}{c|ccccc}
    % % 	\toprule
    % \whline
    % 	 \textbf{Method} & \textbf{Eff-b0} & \textbf{Eff-b1} & \textbf{Mob-v3} & \textbf{R-18} & \textbf{R-34 }\\
    % % 	 \midrule
    % \hline
 	  % %   MoCo-V2 & 46.8 & 48.4 & 36.2 & 52.2 & 56.8\\
    %     %  MoCo-V2 + DisCo & 65.6 & 65.8& 64.4 & 60.6 & 62.5\\
    %      SwAV \cite{caron2020unsupervised} & 46.8 & & 19.4 & 60.5 & 63.3\\
    %      SwAV + DisCo & 62.4 & & 55.7 & 60.2 & 63.3\\
    %     %  \bottomrule

==> tables/limited-labels.tex <==
\begin{table}[t]
    \centering
    \caption{ImageNet-1k Top-1 accuracy for self-supervised evaluations using 1\% , 10\% of the annotations for linear fine-tuning, in comparison with the fully supervised linear evaluation baseline. }
    \begin{tabular}{cc|ccc}
    	\toprule
    	 Teacher & Model & 1\% & 10\% & 100\% \\
    	 \midrule
    	 \multirow{9}{*}{R50} & MoCov2 & 25.1 & 41.7 & 42.2\\
    	 & SEED & 38+ & 52+ & 60+ \\
         & Eff-b0 & 41.7 & 56.6 & 66.5\\
        %  \cdashline{2-5}
    % 	 & MoCoV2 & 26.6& 42.5& 48.3\\
        %  & Eff-b1 & 42.1&  56.0& 66.6\\
         \cdashline{2-5}
    	 & MoCov2 & 30.4 & 43.9 & 52.2\\
    	 & SEED & 39+ & 49+ & 57+ \\
         & R-18 & 39.2 & 50.3 &  60.6\\
         \cdashline{2-5}
    	 & MoCov2 & 20.3 & 32.3 & 36.2\\
    	 & SEED & 36+ & 52+ & 55+ \\
         & Mob-v3 & 38.7 & 51.6 &  64.4\\
         \hline
    	 \multirow{6}{*}{R101} & SEED & 40+ & 55+ & 62+\\
         & Eff-b0 & 45.3 & 59.1 & 68.9\\
         \cdashline{2-5}
    	 & SEED & 41+ & 51+ & 55+\\
         & R-18 & 42.0 & 52.0 & 62.3\\
         \cdashline{2-5}
    	 & SEED & 38+ & 51+ & 55+\\
         & Mob-v3 & 41.8 & 53.6 & 65.7\\
         \hline
    	 \multirow{6}{*}{R152} & SEED & 40+ & 56+ & 64+\\
         & Eff-b0 &  51.6 & 63.1 & 67.8\\
         \cdashline{2-5}
    	 & SEED & 42+ & 52+ & 55+\\
         & R-18 & 47.1 & 54.8 & 65.5 \\
         \cdashline{2-5}
    	 & SEED & 40+ & 51+ & 61+\\
         & Mob-v3 & 42.8 & 54.7 & 62.5\\
         \bottomrule
    \end{tabular}
    \label{tab:limited-labels}
\end{table}

==> tables/mlp-hidden-param.tex <==
\begin{table}[tb]
    \centering
    \caption{Parameters for backbone with different dimension of projection head.}
    \begin{tabular}{c|ccccc}
    	\toprule
    	 Dimension & Eff-b0 & Eff-b1 & Mob-v3 & R-18 & R-34 \\
    	 \midrule
    	 0 & 4.0 & 6.4 & 4.2 & 10.7 &  20.4\\
         512 & 4.5 & 6.9 & 4.7 & 11.0 & 20.6\\
         1024 & 5.2 & 7.6 & 5.4 & 11.3 & 20.9\\
         1280 & 5.5 & 7.9 & 5.7 & 11.4 & 21.1\\
         2048 & 6.6 & 9.0 & 6.8 & 11.9 & 21.6\\
         \bottomrule
    \end{tabular}
    \label{tab:mlp-hidden-param}
\end{table}

==> tables/mlp-hidden.tex <==
\begin{table}[t]
    \centering
    \caption{Linear evaluation on ImageNet(Top-1) of representations with different dimension of projection head.}
    % 上面部分是我们的方法，下面是直接MoCo出来finetune的结果
    \begin{tabular}[width=1.0\linewidth]{cc|ccccc}
    	\toprule
    	 Method & D & Eff-b0 & Eff-b1 & Mob-v3 & R-18 & R-34 \\
    	 \midrule
    	 %\multirow{4}{*}{MoCoV2} & 0 & 30.6 & 34.5 & 30.3 & 44.2 & 49.2\\
         %& 512 & 44.9 & 47.0 & 34,7 & 52.6 & 56.8\\
         %& 1024 & 46.5 & 48.4 & 35.7 & 53.8 & 58.2\\
         %& 1280 & 46.8 & 48.4 & \textbf{36.2} & 54.0 & 58.3 \\
         %& 2048 & \textbf{47.8} & \textbf{49.9} & \textbf{36.2} & \textbf{57.0} & \textbf{59.2}\\
         %\midrule
    	 \multirow{4}{*}{Ours} & 0& 59.3& 59.8 & 60.3 & 52.5 & 55.1\\
         & 512 & 62.5 & 62.7 & 62.8 & 57.1 & 58.9\\
         & 1024 & 65.0 & 65.0 & 63.8& 59.2 & 61.3\\
         & 1280 & 65.6 & 65.8 & 63.7 & 59.9 & 61.6 \\
         & 2048 & \textbf{66.5} & \textbf{66.6}& \textbf{64.4} & \textbf{60.6}& \textbf{62.5}\\
         \bottomrule
    \end{tabular}
    \label{tab:mlp-hidden}
\end{table}

==> tables/teachertype.tex <==
\begin{table}[ht]
    \centering
    % \vspace{-15pt}
    \caption{Linear evaluation top-1 accuracy (\%) on ImageNet with variants of teacher pre-training methods. All the teachers are ResNet-50 and the first row is student trained by MoCo-V2 directly without distillation, which is  baseline.}
    % \vspace{5pt}
    % \setlength{\tabcolsep}{1.5mm}{ 
    \begin{tabular}{cc|cccc}
    % 	\toprule
    % 	\whline
    \toprule
    	\multicolumn{2}{c|}{\textbf{Teacher}} & \multicolumn{4}{c}{\textbf{Student}}\\
    	\hline
    	 \textbf{Method} & \textbf{Acc} & \textbf{Eff-b0} & \textbf{Eff-b1} &\textbf{ Mob-v3} & \textbf{R-18} \\
    % 	 \midruleo
    \hline
         - & - & 46.8 & 48.4 & 36.2 & 52.2\\
         \cdashline{1-6}
    	 MoCo-V2 & 67.4 & 66.5 & 66.6 & 64.4& 60.6 \\
         SeLa-V2  71.8 & 62.2 & 68.2 & 66.2 & 64.1 \\
%         %  DCv2 \cite{caron2018deep} & 75.2 & \textcolor{red}{55.2} & \textcolor{red}{64.9} & 65.4 & 65.3 & 64.8\\
         SwAV & 75.3 & 70.0 & 72.1 & 65.0 & 65.1 \\
        %  \whline
        \bottomrule
        %  \bottomrule
    \end{tabular}
    % }
    \label{tab:teachertype}
    % \vspace{-22pt}
\end{table}

% \begin{table*}[ht]
%     \centering
%     \vspace{-5pt}
%     \caption{Linear evaluation top-1 accuracy (\%) on ImageNet with variants of teacher pre-training methods. All the teachers are ResNet-50 and the first row is student trained by MoCo-V2 directly without distillation, which is  baseline.}
%     \vspace{-5pt}
%     % \setlength{\tabcolsep}{1.5mm}{ 
%     \begin{tabular}{cc|ccccc}
%     % 	\toprule
%     	\whline
%     	\multicolumn{2}{c|}{\textbf{Teacher}} & \multicolumn{5}{c}{\textbf{Student}}\\
%     	\hline
%     	 \textbf{Method} & \textbf{Acc} & \textbf{Eff-b0} & \textbf{Eff-b1} &\textbf{ Mob-v3} & \textbf{R-18} & \textbf{R-34} \\
%     % 	 \midruleo
%     \hline
%          - & - & 46.8 & 48.4 & 36.2 & 52.2 & 56.8\\
%          \cdashline{1-7}
%     	 MoCo-V2 \cite{chen2020mocov2} & 67.4 & 66.5 & 66.6 & 64.4& 60.6 & 62.5\\
%          SeLa-V2 \cite{asano2020self} & 71.8 & 62.2 & 68.2 & 66.2 & 64.1 & 65.3\\
%         %  DCv2 \cite{caron2018deep} & 75.2 & \textcolor{red}{55.2} & \textcolor{red}{64.9} & 65.4 & 65.3 & 64.8\\
%          SwAV \cite{caron2020unsupervised} & 75.3 & 70.0 & 72.1 & 65.0 & 65.1 & 67.5\\
%          \whline
%         %  \bottomrule
%     \end{tabular}
%     % }
%     \label{tab:teachertype}
%     \vspace{-13pt}
% \end{table*}

==> tables/transfer-cifar.tex <==
% Modify
\begin{table}[t]
    \centering
    \caption{: ImageNet-1k Accuracy (\%) of student network (EfficientNet-B0 and ResNet-18) transferred to other domains (CIFAR-10, CIFAR-100) with and without distillation from lager architectures ResNet-50.}
    \begin{tabular}{ccc|cc}
        \toprule
         Dataset &  Method & Teacher & Eff-b0 & R-18 \\
         \midrule
         \multirow{3}{*}{Cifar10} & MoCo-V2 & \multirow{3}{*}{R-50}& 78.0 & 80.6 \\
          & SEED & & 87.0 & 82.5 \\
          & ours & & \textbf{91.5} & \textbf{85.2} \\
         \multirow{2}{*}{Cifar10} & SEED & \multirow{2}{*}{R-101} & 88.5+ & 83+ \\
          & ours & & 92.2 & 87.3 \\
         \multirow{2}{*}{Cifar10} & SEED & \multirow{2}{*}{R-152}& 88.5+ & 84.5+ \\
          & ours & & 93.5 & 88.1 \\
          \cdashline{1-5}
         \multirow{3}{*}{Cifar100} & MoCo-V2 & \multirow{3}{*}{R-50} & 57.4 & 48.3 \\
          & SEED & & 63.0 & 57.2 \\
          & ours & &\textbf{ 73.2} & \textbf{63.8} \\
         \multirow{2}{*}{Cifar100} & SEED & \multirow{2}{*}{R-101} & 64+ & 57+ \\
          & ours & & 73.4 & 67.4 \\
         \multirow{2}{*}{Cifar100} & SEED & \multirow{2}{*}{R-152} & 64+ & 60+ \\
          & ours & & 78.7 & 67.7 \\
         \bottomrule
    \end{tabular}
    \label{tab:transfer-cifar}
\end{table}

% MoCoV2
% 1) small model ssl on ImageNet
% 2) small model finetune last fc on cifar10/100

==> tables/vittabs.tex <==
\begin{table}[ht]
    \centering
    % \vspace{-5pt}
    \caption{Linear evaluation top-1 accuracy (\%) on ImageNet with DINO as testbed. }
    \vspace{2pt}
    \small
    \setlength{\tabcolsep}{1.2mm}{ 
    \begin{tabular}{cc|ccccc}
    % 	\toprule
    	\whline
    	\multicolumn{2}{c|}{\textbf{Teacher}} & \multicolumn{5}{c}{\textbf{Student}}\\
    	\hline
    	 \textbf{Model} & \textbf{Acc} & \textbf{ViT-tiny} & \textbf{XCiT-tiny}  \\
    % 	 \midruleo
    \hline
         - & - & 63.2 & 67  \\
         \cdashline{1-7}
    	 ViT-small \cite{dosovitskiy2020image,touvron2021training} & 77 & 68.4\greenp{5.2$\uparrow$} & - \\
         XCiT-small \cite{el2021xcit} & 77.8 & - & 71.1\greenp{4.1$\uparrow$}  \\
         \whline
        %  \bottomrule
    \end{tabular}}
    \label{tab:vittabs}
    % \vspace{-13pt}
\end{table}
